Equilibrium States for Non-Uniformly Expanding Skew Products

We study equilibrium states for non-uniformly expanding skew products, and show how a family of fiberwise transfer operators can be used to define the conditional measures along fibers of the product. We prove that the pushforward of the equilibrium state onto the base of the product is itself an equilibrium state for a H\"older potential defined via these fiberwise transfer operators.

==> Phi_Holder.tex <==


\begin{lemma}
There exists $C_2>0$ such that $|\Phi_n(x)-\Phi_n(x')|\leq C_2\ d_n(x,x')^\alpha$.
\label{sec:cont}
\end{lemma}

\begin{proof}
Let $n\geq 0$ and $d_n(x,x')<\delta_0\footnote{define $\delta_0$..}$. Fix $\psi\in \Lambda_K$ and $y\in Y$. Then
\begin{align*}
    \LL_x^{n}\psi(x_{n},y)&=\sum_{\overline{y}\in g_x^{-n}y}e^{S_n\varphi(x,\overline{y})}\psi(x,\overline{y}) \\
    &\leq e^{\big(K_0\sum_{i=1}^k\gamma^{-\alpha i}+K\gamma^{-\alpha n}\big)d(x_n,x_n')^\alpha}\sum_{y'\in g_{x'}^{-(n+1)}y}e^{S_n\varphi(x',\overline{y}')}\psi(x',\overline{y}').
\end{align*} Define $K_n=K_0\sum_{i=1}^k\gamma^{-\alpha i}+K\gamma^{-\alpha n}$, we get \[\Bigg|\log\dfrac{\LL_x^n\psi(x_n,y)}{\LL_{x'}^{n}\psi(x'_n,y)}\Bigg|\leq K_n\ d(x_n,x'_n)^\alpha.\]

Consider $\Phi$ defined with respect to $\delta_y$, the delta measure at $y$. 
\begin{align*}
\big|\Phi_n(x)-\Phi_n(x')\big|&=\Bigg|\log\dfrac{\LL_x^{n+1}(x_{n+1},y)\LL_{fx'}^n(x_{n+1},y)}{\LL_{fx}^n(x_{n+1},y)\LL_{x'}^{n+1}(x_{n+1},y)}\Bigg|\\
&\leq \Bigg|\log\dfrac{\LL_x^{n+1}(x_{n+1},y)}{\LL_{x'}^{n+1}(x_{n+1},y)}\Bigg|+\Bigg|\log\dfrac{\LL_{fx'}^n(x_{n+1},y)}{\LL_{fx}^n(x_{n+1},y)}\Bigg|\\
&\leq (K_{n+1}+K_{n})\ d(f^{n+1}x,f^{n+1}x')^\alpha\\
&\leq (K_{n+1}+K_{n})\Gamma^\alpha\ d(x_{n},x'_{n})^\alpha.
\end{align*} where the third line holds by Lemma~\ref{sec:ratio} and the  last by the inherited Lipschitz condition for $f$. Note that $K_n\to\dfrac{K_0}{1-\gamma^{-\alpha}}$ as $n\to\infty$. Then for any $B>\dfrac{K_0}{1-\gamma^{-\alpha}}$, there exists $N$ such that $K_n<B$ for all $n\geq N$. Thus, for $n\geq N$ \[\big|\Phi_n(x)-\Phi_n(x')\big|\leq 2B\Gamma^\alpha\ d(x_{n},x'_{n})^\alpha\leq 2B\Gamma^\alpha\ d_n(x,x')^\alpha.\]

\end{proof}

\begin{theorem}
The potential $\Phi$ constructed in Theorem~\ref{sec:potential} is $\alpha$-$\holder$ continuous.
\label{thm:PhiHolder}
\end{theorem}

\begin{proof}
Let $C=\max\{C_1,C_2\}$. For any $n\geq0$, \begin{align*}
    \big|\Phi(x)-\Phi(x')\big|&\leq \big|\Phi(x)-\Phi_n(x)\big|+\big|\Phi_n(x)-\Phi_n(x')\big|+\big|\Phi_n(x')-\Phi(x')\big|\\
    &\leq 2C\tau^n+Cd_n(x_n,x'_n)^\alpha\\
    &\leq 2C\tau^n+C\Gamma^{\alpha n}d(x,x')^\alpha
\end{align*} where the second inequality follows from Lemma~\ref{sec:potential} and Lemma~\ref{sec:cont}. Choose $N\in \NN$ so that $\tau^N\leq \Gamma^{\alpha N}d(x,x')^\alpha$. Then \[ \big|\Phi(x)-\Phi(x')\big|\leq 3C\Gamma^{\alpha N}d(x,x')^\alpha\] which finishes the proof.
\end{proof}
